Supernova search with active learning in ZTF DR3

We provide the first results from the complete SNAD adaptive learning pipeline in the context of a broad scope of data from large-scale astronomical surveys. The main goal of this work is to explore the potential of adaptive learning techniques in application to big data sets. Our SNAD team used Active Anomaly Discovery (AAD) as a tool to search for new supernova (SN) candidates in the photometric data from the first 9.4 months of the Zwicky Transient Facility (ZTF) survey, namely, between March 17 and December 31 2018 (58194 < MJD < 58483). We analysed 70 ZTF fields at a high galactic latitude and visually inspected 2100 outliers. This resulted in 104 SN-like objects being found, 57 of which were reported to the Transient Name Server for the first time and with 47 having previously been mentioned in other catalogues, either as SNe with known types or as SN candidates. We visually inspected the multi-colour light curves of the non-catalogued transients and performed fittings with different supernova models to assign it to a probable photometric class: Ia, Ib/c, IIP, IIL, or IIn. Moreover, we also identified unreported slow-evolving transients that are good superluminous SN candidates, along with a few other non-catalogued objects, such as red dwarf flares and active galactic nuclei. Beyond confirming the effectiveness of human-machine integration underlying the AAD strategy, our results shed light on potential leaks in currently available pipelines. These findings can help avoid similar losses in future large-scale astronomical surveys. Furthermore, the algorithm enables direct searches of any type of data and based on any definition of an anomaly set by the expert.

==> AAD_SN_A&A(2)/table.tex <==
% \label{sec:appendix-outliers}
% \onecolumn
    % \begin{landscape}
    % \begin{longtable}{lccccclll}
    \begin{longtable}{p{0.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{2.5cm}p{1.2cm}p{2.2cm}p{2.6cm}p{2.5cm}}
        \caption{A complete list of supernovae and supernova candidates found by active anomaly discovery algorithm in ZTF DR3.}
      \label{tab:sn_list}
      \\
\hline
№	&	Name	&	R.A.	&	Dec.	&	OID	&	Type$^*$	&	\maria{Target alert name}	&	Other names	&	Remarks	\\
1	&	SNAD101	&	247.45543	&	24.77282	&	633207400004730	&	IIn	&	ZTF18abqkqdm	&	AT 2018lwh	&	\\
2	&	SNAD102	&	245.05375	&	28.38220	&	633216300024691	&	IIn	&	ZTF18abdgwos	&	AT 2018lwi	&	\\
3	&	SNAD103	&	219.83787	&	47.40378	&	758205100001118	&	IIP	&		&	AT 2018lwj	&	\\
4	&	SNAD104	&	218.91620	&	46.38441	&	758205400019523	&	IIP	&	ZTF18aawqbuc	&	AT 2018lwk	&	\\
5	&	SNAD105	&	218.34626	&	49.22553	&	758209200010983	&	Ibc	&		&	AT 2018lwl	&	\\
6	&	SNAD106	&	219.41935	&	50.16706	&	758213400002862	&	Ia	&		&	AT 2018lwm	&	\\
7	&	SNAD107	&	254.41703	&	44.29804	&	762202300014913	&	Ibc	&		&	AT 2018lwn	&   \\
8	&	SNAD108	&	257.84004	&	48.21127	&	762209400037712	&	Ia	&	ZTF18abauopo	&	AT 2018lwo	&	\\
9	&	SNAD109	&	191.17808	&	54.31252	&	790207100016149	&	IIn	&		&	AT 2018lwp	&	\\
10	&	SNAD111	&	263.42634	&	52.62203	&	796201100002136	&	Ibc	&	ZTF18abdldos	&	AT 2018lwr	&	\\
11	&	SNAD112	&	263.37725	&	51.25848	&	796201400007564	&	Ia	&	ZTF18aaubejv	&	AT 2018lws	&	\\
12	&	SNAD113	&	254.81890	&	58.37547	&	796215200010831	&	Ia	&	ZTF18abmmdnx	&	AT 2018lwt	&	825204400024382	\\
13	&	SNAD113	&	254.81983	&	58.37536	&	825204400024382	&	Ia	&	ZTF18abmmdnx	&	AT 2018lwt	&	796215200010831	\\
14	&	SNAD114	&	257.27308	&	57.55380	&	796215400002705	&	IIn	&	ZTF18aawkaod	&	AT 2018lwu	&	\\
15	&	SNAD115	&	252.82337	&	62.83286	&	824209400038197	&	IIn	&	ZTF18absufwv	&	AT 2018lwv	&	\\
16	&	SNAD116	&	242.29542	&	62.48738	&	824212400005043	&	Ia	&	ZTF18abklrmo	&	AT 2018lww	&	\\
17	&	SNAD117	&	254.04870	&	65.01217	&	824213100016761	&	IIP	&	ZTF18aanbiig	&	AT 2018lwx	&	\\
18	&	SNAD119	&	245.80060	&	68.69152	&	847207200014161	&	IIn	&	ZTF18abgujpm	&	AT 2018lwz	&	\\
19	&	SNAD120	&	255.06791	&	70.51376	&	847209200012956	&	IIP	&	ZTF18aazydub	&	AT 2018lxa	& 	\\
20	&	SNAD121	&	248.33307	&	71.11514	&	847211100017171	&	IIP	&	ZTF18abklshn	&	AT 2018lxb	&	\\
21	&	SNAD122	&	217.38363	&	33.54185	&	676212400013135	&	IIP	&	ZTF18aawqcqz	&	AT 2018lxg	&	\\
22	&	SNAD123	&	230.71268	&	41.05182	&	720209400014960	&	IIn	&	ZTF18aagrczj	&	AT 2018lxh	&	721212300003198	\\
23	&	SNAD123	&	230.71268 	&	41.05184	&	721212300003198	&	IIn	&	ZTF18aagrczj	&	AT 2018lxh	&	720209400014960	\\
24	&	SNAD124	&	212.14042	&	58.49805	&	792215100001492	&	IIL	&	ZTF18aaigpcr	&	AT 2018lxi	&	821201400006340	\\
25	&	SNAD124	&	212.14043	&	58.49805	&	821201400006340	&	IIL	&	ZTF18aaigpcr	&	AT 2018lxi	&	792215100001492	\\
26	&	SNAD125	&	222.74691	&	55.19418	&	793211300013937	&	Ia	&	ZTF18aaykuzt	&	AT 2018lxj	&	\\
27	&	SNAD126	&	226.65118	&	54.70207	&	793206100016155	&	IIn	&	ZTF18aaziehk	&	AT 2018lxk	&	\\
28	&	SNAD127	&	224.96223	&	57.52264	&	793214300002434	&	IIn	&	ZTF18aaqufmy	&	AT 2018lxl	&	\\
29	&	SNAD128	&	230.50802 	&	53.61611	&	793205400010761	&	IIn	&		&	AT 2018lxm	&	\\
30	&	SNAD129	&	237.28114 	&	41.91548	&	721210100012349	&	IIL	&	ZTF18aalrsbd 	&	AT 2018lxn	&	\\
31	&	SNAD130	&	232.13026 	&	51.98997	&	794204400017737	&	Ia	&	ZTF18abedlru	&	AT 2018lxo	&	\\
32	&	SNAD131	&	239.69206 	&	56.42458	&	794209200012381	&	Ibc	&		&	AT 2018lxp	&	\\
33	&	SNAD132	&	239.95822 	&	55.34216	&	794209300004376	&	Ibc	&	ZTF18aaumixp	&	AT 2018lxq	&	\\
34	&	SNAD133	&	242.93762 	&	55.96133	&	795212100007964	&	Ia	&	ZTF18aanbksg	&	AT 2018lxr	&	\\
35	&	SNAD134	&	252.30216 	&	54.11178	&	795205100007271	&	Ia	&	ZTF18aayatjf	&	AT 2018lxs	&	\\
36	&	SNAD135	&	242.30742 	&	52.21426	&	795204100013041	&	IIn	&	ZTF18abgvctp 	&	AT 2018lxt	&	\\
37	&	SNAD136	&	257.67202	&	 63.69693	&	825211200009477	&	Ia	&	ZTF18abrwswl 	&	AT 2018lxu	&	\\
38	&	SNAD137	&	260.16229	&	 59.49770	&	825202200039582	&	IIn	&	ZTF18aaqzcvy	&	AT 2018lxv	&	\\
39	&	SNAD138	&	257.88902 	&	62.49717	&	825211300010764	&	Ia	&	ZTF18abedwws 	&	AT 2018lxw	&	\\
40	&	SNAD139	&	264.55471 	&	44.26862	&	763202300013915	&	IIn	&	ZTF18aajtpsk	&	AT 2018lxx	&	\\
41	&	SNAD141	&	268.46498 	&	70.79590	&	848210200003752	&	Ia	&		&	AT 2018lxz	&	\\
42	&	SNAD142	&	274.19431 	&	59.44037	&	826202200030732	&	IIP	&	ZTF18ablvrgt	&	AT 2018lya	&	\\
43	&	SNAD143	&	270.03210 	&	34.66995	&	682209200018910	&	IIP	&	ZTF18aaqzrpf	&	AT 2018lyb	&	\\
44	&	SNAD144	&	269.87561 	&	49.88876	&	764216400008221	&	Ia	&	ZTF18abwlrdj	&	AT 2018lyc	&	\\
45	&	SNAD145	&	275.79452	&	48.31019	&	764210400028832	&	Ibc	&		&	AT 2018lyd	&	\\
46	&	SNAD146	&	197.21596	&	44.96981	&	756202100006670	&	IIn	&	ZTF18aahiqfy	&	AT 2018lyr	&	\\
47	&	SNAD147	&	192.55741	&	46.63066	&	756207300010654	&	IIn	&		&	AT 2018lys	&	\\
48	&	SNAD160	&	205.97232	&	61.55479	&	821207100004043	&	IIP	&	 ZTF18aautopz	&	AT 2018lzi	&	\\
49	&	SNAD161	&	200.90323	&	55.97815	&	791211100013499	&	Ibc	&	ZTF19aaroswc	&	AT 2018lzj	&	\\
50	&	SNAD162	&	267.30305	&	62.14472	&	825209400016106	&	Ia	&		&	AT 2018lzk	&	\\
51	&	SNAD163	&	265.04514	&	58.79008	&	825201300004134	&	Ibc	&		&	AT 2018lzl	&	\\
52	&	SNAD164	&	274.46930	&	62.62716	&	826210300004963	&	Ia	&	ZTF18abnwqje	&	AT 2018lzm	& \\
53	&	SNAD165	&	259.39972	&	44.51506	&	763204300004087	&	Ibc	&		&	AT 2018lzn	& \\
54	&	SNAD166	&	259.60178	&	48.60846	&	763212400008960	&	Ia	&	ZTF18abrwtqb	&	AT 2018lzo	&	\\
55	&	SNAD184	&	223.60115	&	32.77872	&	676205100003608	&	IIL	&	ZTF18abdgucl	&	AT 2018mby	&	\\
56	&	SNAD185	&	191.47409	&	42.22174	&	716211100008498	&	IIL	&	ZTF18acnnerq	&	AT 2018mbz	&	\\
57	&	SNAD186	&	204.74466	&	43.90742	&	718216200026001	&	IIL	&	ZTF18aagrfaw	&	AT 2018mca	&	\\
58	&	SNAD187	&	208.28069	&	40.80206	&	718211400012193	&	IIP	&	ZTF18aaqctvg	&	AT 2018mcb	&	\\
59	&	SNAD188	&	210.69041	&	39.65870	&	718206100007526	&	Ia	&		&	AT 2018mcc	& 	\\
60	&	SNAD189	&	224.46669	&	38.95331	&	720207300005154	&	Ia	&		&	AT 2018mcd	& 	\\
61	&		&	246.05583	&	25.27213	&	633208100018991	&	Ia-91bg 	&	ZTF18aaiajvb	&	SN 2018baz	&		\\
62	&		&	252.75330	&	25.87635	&	634208100013151	&	Ia	&	ZTF18abmxfrc	&	SN 2018fin	&		\\
63	&		&	256.52059	&	29.66854	&	634214200012529	&	II	&	ZTF18aainvic	&	SN 2018jo	&		\\
64	&		&	224.06941	&	34.05073	&	676209400030690	&	PSN	&	ZTF18aalsomy	&	AT 2018cff	&		\\
65	&		&	266.98595	&	34.93270	&	682210200032862	&	PSN	&	ZTF18aamlqqh	&	AT 2018bcz	&		\\
66	&		&	264.50123	&	35.08437	&	682212100012973	&	PSN	&		&	AT 2018bhu	&		\\
\multirow{2}{*}{67}	&		&	212.59125	&	39.32474	&	718205300001790	&	PSN	&	ZTF18aacckja	&	\small{MASTER OT}	&		\\
	&		&		&		&		&		&		&	\small{J141021.86+391928.4}	&		\\
\multirow{2}{*}{68}	&		&	213.91916	&	43.53175	&	718213100006185	&	PSN	&	ZTF18aaihqtg	&	\small{MLS180418:}	&	719216200005369	\\
	&		&		&		&		&		&		&	\small{141541+433154}	&		\\
69	&		&	218.33353	&	41.26712	&	719210300033956	&	Ib	&	ZTF18aagrdcs	&	SN 2018alc	&		\\
\multirow{2}{*}{70}	&		&	213.91894	&	43.53171	&	719216200005369	&	PSN	&	ZTF18aaihqtg	&	\small{MLS180418:}	&	718213100006185	\\
	&		&		&		&		&		&		&	\small{141541+433154}	&		\\
71	&		&	226.84514	&	38.41658	&	720202200013161	&	Ia	&	ZTF18aabyhlc	&	SN 2018aab	&		\\
72	&		&	232.22274	&	37.62043	&	721204400000387	&	PSN	&	ZTF18aaikozr	&	AT 2018doz	&		\\
73	&		&	237.51483	&	42.08853	&	721210100010621	&	Ia	&	 ZTF18aagstdc	&	SN 2018apn	&		\\
74	&		&	247.27265	&	39.88654	&	722205200035190	&	II	&	ZTF18aalbpll	&	SN 2018cbb	&		\\
75	&		&	245.78265	&	39.31497	&	722206400011527	&	II	&	ZTF18aahbfcr	&	SN 2018anx	&		\\
76	&		&	247.26026	&	43.62678	&	722213200005805	&	II	&	ZTF18aarpttw	&	SN 2018bqs	&		\\
77	&		&	248.04807	&	42.71343	&	722213400026577	&	Ia	&	ZTF18aagtcxj	&	SN 2018aqm	&		\\
78	&		&	254.27082	&	39.38169	&	723206400011620	&	IIP	&	ZTF18aajczsi	&	SN 2018aql	&		\\
79	&		&	248.97523	&	40.03282	&	723208100004162	&	II	&	ZTF18aaiyqow	&	SN 2018gk	&		\\
80	&		&	247.27265	&	39.88654	&	723211300005112	&	Ic BL	&	ZTF18abukavn	&	SN 2018gep	&		\\
81	&		&	250.36668	&	44.02829	&	723215200033236	&	PSN	&	ZTF18abitwua	&	AT 2018feo	&	762204400033332	\\
82	&		&	251.97713	&	42.96844	&	723215400005033	&	Ia	&	ZTF18abpmmpo	&	SN 2018fnd	&		\\
83	&		&	240.45421	&	47.39072	&	761208100023231	&	Ia	&	ZTF18aamlhee	&	SN 2018zs	&		\\
84	&		&	254.72370	&	45.28910	&	762202200038305	&	Ic	&	ZTF18abfzhct	&	SN 2018dxt	&		\\
85	&		&	252.70920	&	45.39807	&	762203100020850	&	II	&	ZTF18abffyqp	&	SN 2018dfi 	&		\\
86	&		&	250.36654	&	44.02827	&	762204400033332	&	PSN	&	ZTF18abitwua	&	AT 2018feo	&	723215200033236	\\
87	&		&	254.77103	&	47.23657	&	762206200028741	&	Ia	&	ZTF18abauprj	&	SN 2018cnw	&		\\
\multirow{2}{*}{88}		&		&	259.28671	&	48.03253	&	763212400019431	&	PSN	&	ZTF18aarrffk	&	\small{MLS180604:}	&		\\
	&		&		&		&		&		&		&	\small{171709+480157}	&		\\
89	&		&	265.56735	&	50.48871	&	763214400010041	&	II	&	ZTF18aamiman	&	SN 2018arc	&		\\
90	&		&	185.39255	&	55.57447	&	789209400002035	&	Ia	&	ZTF18aaiscil 	&	SN 2018aae	&	790212300001679	\\
91	&		&	185.39253	&	55.57446	&	790212300001679	&	Ia	&	ZTF18aaiscil 	&	SN 2018aae	&	789209400002035	\\
92	&		&	203.77313	&	53.87516	&	791206300017767	&	Ia	&	ZTF18aakecej	&	SN 2018bbj	&		\\
93	&		&	200.67064	&	54.35235	&	791207200004054	&	PSN	&	ZTF18aaitbcm	&	AT 2018awa	&		\\
\multirow{2}{*}{94}	&		&	208.78603	&	58.49483	&	791213100013510	&	SLSN-I	&	ZTF18aajqcue	&	SN 2018don	&	792216100036120, \\
	&		&		&		&	&		&		&		&	792216100000865	\\
95	&		&	209.77291	&	58.26840	&	792216100002676	&	Ia	&		&	SN 2018avz	&		\\
\multirow{2}{*}{96}	&		&	208.78615	&	58.49533	&	792216100036120	&	SLSN-I	&	ZTF18aajqcue	&	SN2018don	&	791213100013510, \\
	&		&		&		&	&		&		&		&	792216100000865	\\
\multirow{2}{*}{97}	&		&	208.78601	&	58.49476	&	792216100000865	&	SLSN-I	&	ZTF18aajqcue	&	SN2018don	&	791213100013510, \\
	&		&		&		&	&		&		&		&	792216100036120	\\
98	&		&	230.21754	&	54.21590	&	793205100013372	&	IIP	&	ZTF18abcfdzu	&	SN 2018dfa	&	794208200022136	\\
99	&		&	222.69960	&	54.40795	&	793207200003904	&	Ia	&	ZTF18aakglgw	&	SN 2018aoy	&		\\
100	&		&	230.21751	&	54.21591	&	794208200022136	&	IIP	&	ZTF18abcfdzu	&	SN 2018dfa	&	793205100013372	\\
\multirow{2}{*}{101}	&		&	248.65767	&	52.27841	&	795202100005941	&	PSN	&	ZTF18aanbnjh	&	\small{MLS180307:}	&		\\
	&		&		&		&	&		&		&	\small{163438+521642}	&		\\
102	&		&	244.74136	&	56.71714	&	795211200035931	&	Ia	&	ZTF18aazixbw	&	SN 2018coi	&		\\
103	&		&	252.50392	&	55.83982	&	796212200009183	&	PSN	&	ZTF18abrwrch	&	AT 2018giw	&		\\
104	&		&	274.99848	&	51.79623	&	798204300012865	&	IIb	&	ZTF18abgrbjb	&	SN 2018efd	&		\\
105	&		&	277.67808	&	54.63441	&	798207200002997	&	Ia Pec	&	ZTF18abhpgje	&	SN 2018eul	&		\\
106	&		&	197.86570	&	65.63811	&	821216200012526	&	Ic	&	ZTF18aaisyyp	&	SN 2018avk	&		\\
107	&		&	261.41326	&	59.44670	&	825202200015692	&	Ia	&	ZTF18aasdted 	&	SN 2018big	&		\\
108	&		&	261.82509	&	58.65272	&	825202400018278	&	PSN	&	ZTF18aalfqdc	&	AT 2018czw	&		\\
109	&		&	252.90590	&	61.54532	&	825208200022152	&	Ia	&	ZTF18aaxwjmp	&	SN 2018coe	&		\\
110	&		&	271.04939	&	59.81758	&	826203200034373	&	PSN	&	ZTF18aawkdbk	&	AT 2018cjm	&		\\
111	&		&	94.51328	&	78.36701	&	858216400012109	&	IIn	&	ZTF18abtgyme	&	SN 2018zd	&		\\
112	&		&	248.00946	&	78.21141	&	864211100001497	&	IIb	&	ZTF18aaxljll	&	SN 2018gj	&		\\
113	&		&	277.17167	&	75.81321	&	865206200014558	&	Ic	&	ZTF18acapyww	&	SN 2018hpq	&		\\
\hline
% }
\end{longtable}
$^*$For the SNAD candidates type corresponds to the best-fit model according to the fit with Nugent's supernova templates.
% \end{landscape}
% \twocolumn

==> table.tex <==
% \label{sec:appendix-outliers}
% \onecolumn
    % \begin{landscape}
    % \begin{longtable}{lccccclll}
    \begin{longtable}{p{0.3cm}p{1.3cm}p{1.3cm}p{1.3cm}p{2.5cm}p{1.2cm}p{2.2cm}p{2.6cm}p{2.5cm}}
        \caption{A complete list of supernovae and supernova candidates found by active anomaly discovery algorithm in ZTF DR3.}
      \label{tab:sn_list}
      \\
\hline
№	&	Name	&	R.A.	&	Dec.	&	OID	&	Type$^*$	&	\maria{Target alert name}	&	Other names	&	Remarks	\\
1	&	SNAD101	&	247.45543	&	24.77282	&	633207400004730	&	IIn	&	ZTF18abqkqdm	&	AT 2018lwh	&	\\
2	&	SNAD102	&	245.05375	&	28.38220	&	633216300024691	&	IIn	&	ZTF18abdgwos	&	AT 2018lwi	&	\\
3	&	SNAD103	&	219.83787	&	47.40378	&	758205100001118	&	IIP	&		&	AT 2018lwj	&	\\
4	&	SNAD104	&	218.91620	&	46.38441	&	758205400019523	&	IIP	&	ZTF18aawqbuc	&	AT 2018lwk	&	\\
5	&	SNAD105	&	218.34626	&	49.22553	&	758209200010983	&	Ibc	&		&	AT 2018lwl	&	\\
6	&	SNAD106	&	219.41935	&	50.16706	&	758213400002862	&	Ia	&		&	AT 2018lwm	&	\\
7	&	SNAD107	&	254.41703	&	44.29804	&	762202300014913	&	Ibc	&		&	AT 2018lwn	&   \\
8	&	SNAD108	&	257.84004	&	48.21127	&	762209400037712	&	Ia	&	ZTF18abauopo	&	AT 2018lwo	&	\\
9	&	SNAD109	&	191.17808	&	54.31252	&	790207100016149	&	IIn	&		&	AT 2018lwp	&	\\
10	&	SNAD111	&	263.42634	&	52.62203	&	796201100002136	&	Ibc	&	ZTF18abdldos	&	AT 2018lwr	&	\\
11	&	SNAD112	&	263.37725	&	51.25848	&	796201400007564	&	Ia	&	ZTF18aaubejv	&	AT 2018lws	&	\\
12	&	SNAD113	&	254.81890	&	58.37547	&	796215200010831	&	Ia	&	ZTF18abmmdnx	&	AT 2018lwt	&	825204400024382	\\
13	&	SNAD113	&	254.81983	&	58.37536	&	825204400024382	&	Ia	&	ZTF18abmmdnx	&	AT 2018lwt	&	796215200010831	\\
14	&	SNAD114	&	257.27308	&	57.55380	&	796215400002705	&	IIn	&	ZTF18aawkaod	&	AT 2018lwu	&	\\
15	&	SNAD115	&	252.82337	&	62.83286	&	824209400038197	&	IIn	&	ZTF18absufwv	&	AT 2018lwv	&	\\
16	&	SNAD116	&	242.29542	&	62.48738	&	824212400005043	&	Ia	&	ZTF18abklrmo	&	AT 2018lww	&	\\
17	&	SNAD117	&	254.04870	&	65.01217	&	824213100016761	&	IIP	&	ZTF18aanbiig	&	AT 2018lwx	&	\\
18	&	SNAD119	&	245.80060	&	68.69152	&	847207200014161	&	IIn	&	ZTF18abgujpm	&	AT 2018lwz	&	\\
19	&	SNAD120	&	255.06791	&	70.51376	&	847209200012956	&	IIP	&	ZTF18aazydub	&	AT 2018lxa	& 	\\
20	&	SNAD121	&	248.33307	&	71.11514	&	847211100017171	&	IIP	&	ZTF18abklshn	&	AT 2018lxb	&	\\
21	&	SNAD122	&	217.38363	&	33.54185	&	676212400013135	&	IIP	&	ZTF18aawqcqz	&	AT 2018lxg	&	\\
22	&	SNAD123	&	230.71268	&	41.05182	&	720209400014960	&	IIn	&	ZTF18aagrczj	&	AT 2018lxh	&	721212300003198	\\
23	&	SNAD123	&	230.71268 	&	41.05184	&	721212300003198	&	IIn	&	ZTF18aagrczj	&	AT 2018lxh	&	720209400014960	\\
24	&	SNAD124	&	212.14042	&	58.49805	&	792215100001492	&	IIL	&	ZTF18aaigpcr	&	AT 2018lxi	&	821201400006340	\\
25	&	SNAD124	&	212.14043	&	58.49805	&	821201400006340	&	IIL	&	ZTF18aaigpcr	&	AT 2018lxi	&	792215100001492	\\
26	&	SNAD125	&	222.74691	&	55.19418	&	793211300013937	&	Ia	&	ZTF18aaykuzt	&	AT 2018lxj	&	\\
27	&	SNAD126	&	226.65118	&	54.70207	&	793206100016155	&	IIn	&	ZTF18aaziehk	&	AT 2018lxk	&	\\
28	&	SNAD127	&	224.96223	&	57.52264	&	793214300002434	&	IIn	&	ZTF18aaqufmy	&	AT 2018lxl	&	\\
29	&	SNAD128	&	230.50802 	&	53.61611	&	793205400010761	&	IIn	&		&	AT 2018lxm	&	\\
30	&	SNAD129	&	237.28114 	&	41.91548	&	721210100012349	&	IIL	&	ZTF18aalrsbd 	&	AT 2018lxn	&	\\
31	&	SNAD130	&	232.13026 	&	51.98997	&	794204400017737	&	Ia	&	ZTF18abedlru	&	AT 2018lxo	&	\\
32	&	SNAD131	&	239.69206 	&	56.42458	&	794209200012381	&	Ibc	&		&	AT 2018lxp	&	\\
33	&	SNAD132	&	239.95822 	&	55.34216	&	794209300004376	&	Ibc	&	ZTF18aaumixp	&	AT 2018lxq	&	\\
34	&	SNAD133	&	242.93762 	&	55.96133	&	795212100007964	&	Ia	&	ZTF18aanbksg	&	AT 2018lxr	&	\\
35	&	SNAD134	&	252.30216 	&	54.11178	&	795205100007271	&	Ia	&	ZTF18aayatjf	&	AT 2018lxs	&	\\
36	&	SNAD135	&	242.30742 	&	52.21426	&	795204100013041	&	IIn	&	ZTF18abgvctp 	&	AT 2018lxt	&	\\
37	&	SNAD136	&	257.67202	&	 63.69693	&	825211200009477	&	Ia	&	ZTF18abrwswl 	&	AT 2018lxu	&	\\
38	&	SNAD137	&	260.16229	&	 59.49770	&	825202200039582	&	IIn	&	ZTF18aaqzcvy	&	AT 2018lxv	&	\\
39	&	SNAD138	&	257.88902 	&	62.49717	&	825211300010764	&	Ia	&	ZTF18abedwws 	&	AT 2018lxw	&	\\
40	&	SNAD139	&	264.55471 	&	44.26862	&	763202300013915	&	IIn	&	ZTF18aajtpsk	&	AT 2018lxx	&	\\
41	&	SNAD141	&	268.46498 	&	70.79590	&	848210200003752	&	Ia	&		&	AT 2018lxz	&	\\
42	&	SNAD142	&	274.19431 	&	59.44037	&	826202200030732	&	IIP	&	ZTF18ablvrgt	&	AT 2018lya	&	\\
43	&	SNAD143	&	270.03210 	&	34.66995	&	682209200018910	&	IIP	&	ZTF18aaqzrpf	&	AT 2018lyb	&	\\
44	&	SNAD144	&	269.87561 	&	49.88876	&	764216400008221	&	Ia	&	ZTF18abwlrdj	&	AT 2018lyc	&	\\
45	&	SNAD145	&	275.79452	&	48.31019	&	764210400028832	&	Ibc	&		&	AT 2018lyd	&	\\
46	&	SNAD146	&	197.21596	&	44.96981	&	756202100006670	&	IIn	&	ZTF18aahiqfy	&	AT 2018lyr	&	\\
47	&	SNAD147	&	192.55741	&	46.63066	&	756207300010654	&	IIn	&		&	AT 2018lys	&	\\
48	&	SNAD160	&	205.97232	&	61.55479	&	821207100004043	&	IIP	&	 ZTF18aautopz	&	AT 2018lzi	&	\\
49	&	SNAD161	&	200.90323	&	55.97815	&	791211100013499	&	Ibc	&	ZTF19aaroswc	&	AT 2018lzj	&	\\
50	&	SNAD162	&	267.30305	&	62.14472	&	825209400016106	&	Ia	&		&	AT 2018lzk	&	\\
51	&	SNAD163	&	265.04514	&	58.79008	&	825201300004134	&	Ibc	&		&	AT 2018lzl	&	\\
52	&	SNAD164	&	274.46930	&	62.62716	&	826210300004963	&	Ia	&	ZTF18abnwqje	&	AT 2018lzm	& \\
53	&	SNAD165	&	259.39972	&	44.51506	&	763204300004087	&	Ibc	&		&	AT 2018lzn	& \\
54	&	SNAD166	&	259.60178	&	48.60846	&	763212400008960	&	Ia	&	ZTF18abrwtqb	&	AT 2018lzo	&	\\
55	&	SNAD184	&	223.60115	&	32.77872	&	676205100003608	&	IIL	&	ZTF18abdgucl	&	AT 2018mby	&	\\
56	&	SNAD185	&	191.47409	&	42.22174	&	716211100008498	&	IIL	&	ZTF18acnnerq	&	AT 2018mbz	&	\\
57	&	SNAD186	&	204.74466	&	43.90742	&	718216200026001	&	IIL	&	ZTF18aagrfaw	&	AT 2018mca	&	\\
58	&	SNAD187	&	208.28069	&	40.80206	&	718211400012193	&	IIP	&	ZTF18aaqctvg	&	AT 2018mcb	&	\\
59	&	SNAD188	&	210.69041	&	39.65870	&	718206100007526	&	Ia	&		&	AT 2018mcc	& 	\\
60	&	SNAD189	&	224.46669	&	38.95331	&	720207300005154	&	Ia	&		&	AT 2018mcd	& 	\\
61	&		&	246.05583	&	25.27213	&	633208100018991	&	Ia-91bg 	&	ZTF18aaiajvb	&	SN 2018baz	&		\\
62	&		&	252.75330	&	25.87635	&	634208100013151	&	Ia	&	ZTF18abmxfrc	&	SN 2018fin	&		\\
63	&		&	256.52059	&	29.66854	&	634214200012529	&	II	&	ZTF18aainvic	&	SN 2018jo	&		\\
64	&		&	224.06941	&	34.05073	&	676209400030690	&	PSN	&	ZTF18aalsomy	&	AT 2018cff	&		\\
65	&		&	266.98595	&	34.93270	&	682210200032862	&	PSN	&	ZTF18aamlqqh	&	AT 2018bcz	&		\\
66	&		&	264.50123	&	35.08437	&	682212100012973	&	PSN	&		&	AT 2018bhu	&		\\
\multirow{2}{*}{67}	&		&	212.59125	&	39.32474	&	718205300001790	&	PSN	&	ZTF18aacckja	&	\small{MASTER OT}	&		\\
	&		&		&		&		&		&		&	\small{J141021.86+391928.4}	&		\\
\multirow{2}{*}{68}	&		&	213.91916	&	43.53175	&	718213100006185	&	PSN	&	ZTF18aaihqtg	&	\small{MLS180418:}	&	719216200005369	\\
	&		&		&		&		&		&		&	\small{141541+433154}	&		\\
69	&		&	218.33353	&	41.26712	&	719210300033956	&	Ib	&	ZTF18aagrdcs	&	SN 2018alc	&		\\
\multirow{2}{*}{70}	&		&	213.91894	&	43.53171	&	719216200005369	&	PSN	&	ZTF18aaihqtg	&	\small{MLS180418:}	&	718213100006185	\\
	&		&		&		&		&		&		&	\small{141541+433154}	&		\\
71	&		&	226.84514	&	38.41658	&	720202200013161	&	Ia	&	ZTF18aabyhlc	&	SN 2018aab	&		\\
72	&		&	232.22274	&	37.62043	&	721204400000387	&	PSN	&	ZTF18aaikozr	&	AT 2018doz	&		\\
73	&		&	237.51483	&	42.08853	&	721210100010621	&	Ia	&	 ZTF18aagstdc	&	SN 2018apn	&		\\
74	&		&	247.27265	&	39.88654	&	722205200035190	&	II	&	ZTF18aalbpll	&	SN 2018cbb	&		\\
75	&		&	245.78265	&	39.31497	&	722206400011527	&	II	&	ZTF18aahbfcr	&	SN 2018anx	&		\\
76	&		&	247.26026	&	43.62678	&	722213200005805	&	II	&	ZTF18aarpttw	&	SN 2018bqs	&		\\
77	&		&	248.04807	&	42.71343	&	722213400026577	&	Ia	&	ZTF18aagtcxj	&	SN 2018aqm	&		\\
78	&		&	254.27082	&	39.38169	&	723206400011620	&	IIP	&	ZTF18aajczsi	&	SN 2018aql	&		\\
79	&		&	248.97523	&	40.03282	&	723208100004162	&	II	&	ZTF18aaiyqow	&	SN 2018gk	&		\\
80	&		&	247.27265	&	39.88654	&	723211300005112	&	Ic BL	&	ZTF18abukavn	&	SN 2018gep	&		\\
81	&		&	250.36668	&	44.02829	&	723215200033236	&	PSN	&	ZTF18abitwua	&	AT 2018feo	&	762204400033332	\\
82	&		&	251.97713	&	42.96844	&	723215400005033	&	Ia	&	ZTF18abpmmpo	&	SN 2018fnd	&		\\
83	&		&	240.45421	&	47.39072	&	761208100023231	&	Ia	&	ZTF18aamlhee	&	SN 2018zs	&		\\
84	&		&	254.72370	&	45.28910	&	762202200038305	&	Ic	&	ZTF18abfzhct	&	SN 2018dxt	&		\\
85	&		&	252.70920	&	45.39807	&	762203100020850	&	II	&	ZTF18abffyqp	&	SN 2018dfi 	&		\\
86	&		&	250.36654	&	44.02827	&	762204400033332	&	PSN	&	ZTF18abitwua	&	AT 2018feo	&	723215200033236	\\
87	&		&	254.77103	&	47.23657	&	762206200028741	&	Ia	&	ZTF18abauprj	&	SN 2018cnw	&		\\
\multirow{2}{*}{88}		&		&	259.28671	&	48.03253	&	763212400019431	&	PSN	&	ZTF18aarrffk	&	\small{MLS180604:}	&		\\
	&		&		&		&		&		&		&	\small{171709+480157}	&		\\
89	&		&	265.56735	&	50.48871	&	763214400010041	&	II	&	ZTF18aamiman	&	SN 2018arc	&		\\
90	&		&	185.39255	&	55.57447	&	789209400002035	&	Ia	&	ZTF18aaiscil 	&	SN 2018aae	&	790212300001679	\\
91	&		&	185.39253	&	55.57446	&	790212300001679	&	Ia	&	ZTF18aaiscil 	&	SN 2018aae	&	789209400002035	\\
92	&		&	203.77313	&	53.87516	&	791206300017767	&	Ia	&	ZTF18aakecej	&	SN 2018bbj	&		\\
93	&		&	200.67064	&	54.35235	&	791207200004054	&	PSN	&	ZTF18aaitbcm	&	AT 2018awa	&		\\
\multirow{2}{*}{94}	&		&	208.78603	&	58.49483	&	791213100013510	&	SLSN-I	&	ZTF18aajqcue	&	SN 2018don	&	792216100036120, \\
	&		&		&		&	&		&		&		&	792216100000865	\\
95	&		&	209.77291	&	58.26840	&	792216100002676	&	Ia	&		&	SN 2018avz	&		\\
\multirow{2}{*}{96}	&		&	208.78615	&	58.49533	&	792216100036120	&	SLSN-I	&	ZTF18aajqcue	&	SN2018don	&	791213100013510, \\
	&		&		&		&	&		&		&		&	792216100000865	\\
\multirow{2}{*}{97}	&		&	208.78601	&	58.49476	&	792216100000865	&	SLSN-I	&	ZTF18aajqcue	&	SN2018don	&	791213100013510, \\
	&		&		&		&	&		&		&		&	792216100036120	\\
98	&		&	230.21754	&	54.21590	&	793205100013372	&	IIP	&	ZTF18abcfdzu	&	SN 2018dfa	&	794208200022136	\\
99	&		&	222.69960	&	54.40795	&	793207200003904	&	Ia	&	ZTF18aakglgw	&	SN 2018aoy	&		\\
100	&		&	230.21751	&	54.21591	&	794208200022136	&	IIP	&	ZTF18abcfdzu	&	SN 2018dfa	&	793205100013372	\\
\multirow{2}{*}{101}	&		&	248.65767	&	52.27841	&	795202100005941	&	PSN	&	ZTF18aanbnjh	&	\small{MLS180307:}	&		\\
	&		&		&		&	&		&		&	\small{163438+521642}	&		\\
102	&		&	244.74136	&	56.71714	&	795211200035931	&	Ia	&	ZTF18aazixbw	&	SN 2018coi	&		\\
103	&		&	252.50392	&	55.83982	&	796212200009183	&	PSN	&	ZTF18abrwrch	&	AT 2018giw	&		\\
104	&		&	274.99848	&	51.79623	&	798204300012865	&	IIb	&	ZTF18abgrbjb	&	SN 2018efd	&		\\
105	&		&	277.67808	&	54.63441	&	798207200002997	&	Ia Pec	&	ZTF18abhpgje	&	SN 2018eul	&		\\
106	&		&	197.86570	&	65.63811	&	821216200012526	&	Ic	&	ZTF18aaisyyp	&	SN 2018avk	&		\\
107	&		&	261.41326	&	59.44670	&	825202200015692	&	Ia	&	ZTF18aasdted 	&	SN 2018big	&		\\
108	&		&	261.82509	&	58.65272	&	825202400018278	&	PSN	&	ZTF18aalfqdc	&	AT 2018czw	&		\\
109	&		&	252.90590	&	61.54532	&	825208200022152	&	Ia	&	ZTF18aaxwjmp	&	SN 2018coe	&		\\
110	&		&	271.04939	&	59.81758	&	826203200034373	&	PSN	&	ZTF18aawkdbk	&	AT 2018cjm	&		\\
111	&		&	94.51328	&	78.36701	&	858216400012109	&	IIn	&	ZTF18abtgyme	&	SN 2018zd	&		\\
112	&		&	248.00946	&	78.21141	&	864211100001497	&	IIb	&	ZTF18aaxljll	&	SN 2018gj	&		\\
113	&		&	277.17167	&	75.81321	&	865206200014558	&	Ic	&	ZTF18acapyww	&	SN 2018hpq	&		\\
\hline
% }
\end{longtable}
$^*$For the SNAD candidates type corresponds to the best-fit model according to the fit with Nugent's supernova templates.
% \end{landscape}
% \twocolumn
